Bounding the Invertibility of Privacy-preserving Instance Encoding using Fisher Information

Privacy-preserving instance encoding aims to encode raw data as feature vectors without revealing their privacy-sensitive information. When designed properly, these encodings can be used for downstream ML applications such as training and inference with limited privacy risk. However, the vast majority of existing instance encoding schemes are based on heuristics and their privacy-preserving properties are only validated empirically against a limited set of attacks. In this paper, we propose a theoretically-principled measure for the privacy of instance encoding based on Fisher information. We show that our privacy measure is intuitive, easily applicable, and can be used to bound the invertibility of encodings both theoretically and empirically.

==> opt.tex <==
\section{\method: Enforcing Desired dFIL with Practical Utility}
\label{sec:refil}

We propose \method (\textbf{Re}ducing d\textbf{FIL}) as a privacy-enhancing method that enforces the targeted dFIL to a split inference system while maintaining reasonable utility. 
%
From Section~\ref{sec:dfil}, it can be seen that enforcing a specific dFIL can be done by adding a Gaussian noise with $\sigma=\sqrt{\trace(\mathbf{J}_{\mathcal{M}_{client}}^{T}\mathbf{J}_{\mathcal{M}_{client}})/(d * \dfil)}$ to the split layer activation.
%\method calculates the required $\sigma$ for each $\mathbf{x}$ and add it to the activation.
However, achieving smaller dFIL (better privacy) requires adding a larger noise, which can, in turn, hurt the utility of the system.
\method employs two optimizations that can reduce the noise that needs to be added while achieving the same dFIL, to explore a better privacy-utility trade-off.
%\textcolor{red}{TODO: Do we need an algorithm or a figure?}
%From the equations, we can see that increasing $\sigma$ of the added Gaussian noise increases FIB and in turns makes it harder to reconstruct the original input, as expected.

\paragraph{Optimization 1: compression/decompression layer}
The first optimization drops unnecessary information flowing through the split layer by adding a compression layer at the end of the client-side model and a decompression layer at the beginning of the server-side model.
With the compression layer, less noise is required to hide the input, improving the utility.
%
For a compression layer, we use a 1$\times$1 convolution layer of $\phi$: $\mathbb{R}^{c_1\times w\times h} \rightarrow \mathbb{R}^{c_2\times w\times h}$~\cite{splitnets} for CNN, and a fully connected (FC) layer of $\phi$: $\mathbb{R}^{c_1} \rightarrow \mathbb{R}^{c_2}$ for MLP, where $c_1 > c_2$. Similarly, we used a 1$\times$1 convolution layer of $\phi'$: $\mathbb{R}^{c_2\times w\times h} \rightarrow \mathbb{R}^{c_1\times w\times h}$~\cite{splitnets} or a fully connected (FC) layer of $\phi'$: $\mathbb{R}^{c_2} \rightarrow \mathbb{R}^{c_1}$ for decompression. 
%
%They were introduced to reduce the communication overhead in prior split inference literature~\cite{splitnets}.
%
%We observed that adding a compression layer improves the privacy-utility trade-off of \method significantly (Section~\ref{sec:eval_opt}). One explanation is that when a compression layer is added, the model learns to drop unnecessary information flowing throw the split layer, requiring less noise to hide the input.

\paragraph{Optimization 2: SNR loss}
The second optimization directly adds a loss term during the model optimization so that the trained model requires less noise to be added to achieve the same dFIL.
As the noise that needs to be added is $\sigma=\sqrt{\trace(\mathbf{J}_{\mathcal{M}_{client}}^{T}\mathbf{J}_{\mathcal{M}_{client}})/(d * \dfil)}$ for a target dFIL, maximizing the signal-to-noise-ratio (SNR) of the split layer ($\mathbf{z}^T \mathbf{z} / \sigma^2$) is equivalent to minimizing $\trace(\mathbf{J}_{\mathcal{M}_{client}}^{T}\mathbf{J}_{\mathcal{M}_{client}}) / (\mathbf{z}^T \mathbf{z})$.
%
We add the \emph{SNR loss} term to the objective of the training, which trains the model parameters in a way that requires less noise to achieve the same dFIL.
%
Our SNR loss is similar to Jacobian regularizer~\cite{jacobian_regularizer} proposed for robust learning. However, SNR loss differs in that it minimizes the Jacobian \emph{normalized by the activation}.

%Subsampling optimization 
